Memristive Linear Algebra

The advent of memristive devices offers a promising avenue for efficient and scalable analog computing, particularly for linear algebra operations essential in various scientific and engineering applications. This paper investigates the potential of memristive crossbars in implementing matrix inversion algorithms. We explore both static and dynamic approaches, emphasizing the advantages of analog and in-memory computing for matrix operations beyond multiplication. Our results demonstrate that memristive arrays can significantly reduce computational complexity and power consumption compared to traditional digital methods for certain matrix tasks. Furthermore, we address the challenges of device variability, precision, and scalability, providing insights into the practical implementation of these algorithms.

==> secs/Convergence.tex <==
\subsubsection{Potential Issues}
We can write the dynamical equation
\begin{align}
    \frac{dR}{dt}=-\alpha (R-R_\text{off})+\frac{R_\text{on}-R_\text{off}}{\beta}V
\end{align}
and we can try 
\begin{align}
V=\begin{cases} \frac{\beta}{\Delta R}\left(\alpha(-A+I)R-\alpha R_\text{off}+\alpha I \right)
\\
   \frac{\beta}{\Delta R}\alpha(-R_\text{off}+RAR)
\end{cases} .
\end{align}
now we have 
\begin{align}
\frac{dR}{dt}=\begin{cases}
-\alpha(I-AR)
\\
-\alpha R(I-AR)
\end{cases} .
\end{align}

We examine the equilibrium point $(\frac{dR}{dt}=0)$ of both dynamical equations to demonstrate that both solves the inverse matrix problem of interest. In the first case
\begin{align}
    -\alpha R &=-\alpha AR+\alpha R+\alpha I \\
    AR &=I
\end{align}
 and the second case
 \begin{align}
     \alpha R &= \alpha RAR \\
     AR &=I .
 \end{align}

As these potential solve the same dynamical equations we should be able to equate them, thus
\begin{align}
     \frac{\beta}{\Delta R}\left(\alpha(-A+I)R-\alpha R_\text{off}+\alpha I \right)  &\stackrel{?}{=}  \frac{\beta}{\Delta R}\alpha(-R_\text{off}+RAR)
     \\
     -AR+R+I &=RAR \\
     -R^{-1}AR+I+R^{-1} &=AR \\
     -R^{-1}AR+I+R^{-1} &= R+I-RAR \\
     R^{-1}(I-AR)&= R(I-AR)     
\end{align}
thus the potentials are equivalent if $R^{-1}=R$ (and thus $A^{-1}=A$) or $AR=I$, thus these potential are equivalent only at the equilibrium point. We can conclude the potential to approach the equilibrium point and invert the matrix is not unique. 



We can get a sense for the convergence of our dynamical system by examining the stability of the equilibrium solution via a Lyapunov function. If is challenging to find the Lypaunov equation for a non-homogeneous equation, so we begin by looking for a Lyapunov function for the homogeneous solution.

Splitting up our homogenous equations we can identify two Lyapunov functions:
\begin{align}
    \frac{dR}{dt}=-\alpha R \;\; \vert \;\; \mathcal{L}_1=R^2 \\
    \frac{dR}{dt}=\alpha RAR \;\; \vert \;\; \mathcal{L}_2= c AR
\end{align}

We see that $\mathcal{L}_1$ is a well behaved Lyapunov function as $R^2\geq 0$ and $-\alpha 2 R^2$ is non-positive for $\alpha>0$. Similarly we can put constraints on $A$ and $R$ such that $\mathcal{L}_2$ is strictly positive but now we are not guaranteed that $\nabla \mathcal{L}\dot{R}$ is non-positive. 

We can find a candidate Lyaponuv function for the full equation of motion from these forms
\begin{align}
    \frac{dR}{dt} &=-\alpha R +\alpha RAR \;\; \vert \;\; \mathcal{L}=R +AR \\
    \dot{\mathcal{L}} &=\alpha\nabla\mathcal{L}(-R+RAR) \\
    \dot{R}+A\dot{R}&=(I+A)\dot{R}
    \\ &= \alpha(I+A)(-R+RAR)
    \label{eqn:CandidateLyapunov}
\end{align}
Again we see that while $\mathcal{L}$ can be constructed to be strictly positive, but the Lyapunov function is not guaranteed to be non-positive and thus guaranteeing convergence. The right-hand side of the last line of equation \ref{eqn:CandidateLyapunov} is our function which needs to be nonpositive, which is only guaranteed when $AR < I$ if $(I+A)>0$. 

==> secs/SPICE.tex <==
\textcolor{red}{Add picture and explanation of the numerical and the scheme we are using}

==> secs/katz.tex <==
The Katz ranking in social networks is given by
 \begin{equation}
     K = (I-\alpha G)^{-1}\vec 1-\vec  1\ 
 \end{equation}
 where $I$ is the $N\times N$ identity matrix, $\vec 1$ is a $N$-dimensional column vector made of ones.
 This is a typical example of ranking in complex networks, where evaluating an inverse is necessary.

==> secs/onlinereg.tex <==
We now assume that we can perform matrix inversion directly on a chip. Let us now show that with this capability we can also perform online regression. By online regression, we mean the following. As new data is introduced, the memristor values update dynamically to follow the result of a ridge regression.
In particular, let us assume that the data stream is fully time-continuous. This could be for instance the resistance value across a nanowire junction acting as a reservoir.
For instance, the predictors could be the values of the currents or resistances as measured at certain nodes are given by
\begin{eqnarray}
    X_i(t)\equiv \vec x(t)
\end{eqnarray}
where $i$ is a discrete index $i=1\cdots d$, with $d$ the number of predictor values, while $t$ is continuous. We assume we have a teacher signal $Y_\alpha(t)$ with $\alpha=1\cdots m$ as the number of target values. A ridge regression with many discrete observations up to time $t=T$ is given by the minimization of the functional
\begin{eqnarray}
    \text{argmin}_{B} \Big( \|Y-X B\|^2+ \lambda \|B\|^2\Big)
\end{eqnarray}
which, with continuous observation variables is written  as 
\begin{eqnarray}
    \text{argmin}_{B(t)} \Big( \sum_{\alpha=1}^d \int_0^t ds (Y_\alpha(s)-\sum_{j=1}^m X_j (s) B_{j\alpha}(T))^2+ \lambda \sum_{j=1}^m \sum_{\alpha=1}^d B_{j\alpha}(t)^2\Big)
\end{eqnarray}
For fixed horizon $T=t$, the solution of this problem is known and is given by
\begin{eqnarray}
    B_{j\alpha}(t)=\sum_{r=1}^d \Big( \int_0^tds\ X(s)X^{\mathcal T}(s)+\lambda I_{d} \Big)_{jr}^{-1}\int_0^{t}ds X_{r}(s) Y_{\alpha}(s)
\end{eqnarray}
The matrix $B$ has dimensions $d\times m$.
Let us now call $\mathcal M(t)=( \int_0^tds X(s)X^{\mathcal T}(s)+\lambda I_{d} \Big)^{-1}$ and $\mathcal Z(t)=\int_0^{t}ds X_{r}(s) y_{\alpha}(s)$. We also define $\mathcal L(t)=\int_0^tds X(s)X^{\mathcal T}(s)$.
Then, we assume that a memristive circuit is fast enough to evaluate $M(t)$.
Let us assume that we operate a portion of the memristive crossbar of dimension $d\times m$, and that there is still a portion of the crossbar of dimension $d\times d$. Let us call $\mathcal R$ the former portion, and $R$ the latter. We operate the first portion as
\begin{eqnarray}
    \frac{d\mathcal R}{dt}=-\alpha \mathcal A(t) \mathcal R(t)+ \mathcal C(t).
\end{eqnarray}
Let us equate $B(t)\equiv \mathcal R(t)$. Then
\begin{eqnarray}
    \frac{d}{dt} \mathcal R(t)=\frac{d}{dt} \mathcal M(t)\mathcal Z(t)=\frac{d\mathcal M}{dt} \mathcal Z(t)+ \mathcal M(t) \frac{d\mathcal Z}{dt}.
\end{eqnarray}
Note that
\begin{eqnarray}
    \frac{d\mathcal M}{dt}&=&-\mathcal M(t) \mathcal L^\prime (t) \mathcal M(t)\\
    \frac{d\mathcal Z}{dt}&=&X(t) Y(t)
\end{eqnarray}
and thus
\begin{eqnarray}
    \frac{d\mathcal R}{dt}&=&-\mathcal M(t) \mathcal L^\prime (t) \mathcal M(t) \mathcal Z(t)+ \mathcal M(t) X(t) Y(t)\\
    &=&-\mathcal M(t) \mathcal L^\prime (t) \mathcal R(t)+ \mathcal M(t) X(t) Y(t)
\end{eqnarray}
and thus we can identify
\begin{eqnarray}
    \mathcal A(t)&=&\frac{1}{\alpha }\mathcal M(t) \mathcal L^\prime (t)\\
    \mathcal C(t)&=&\mathcal M(t) X(t) Y(t)
\end{eqnarray}
which implies that operating the system as such, with the due assumptions, is in principle able to follow the regression in an online fashion. Note that $\mathcal M(t)^{-1}$ is a positive and invertible matrix, and thus it can be inverted by the algorithm presented earlier.

==> secs/simulbas.tex <==

\subsection{Piecewise Delayed Differential Equation}

We first simulate a simplified model of the system by numerically integrating (1) under a piecewise delayed forcing. We choose $A$ to be a diagonally dominant random matrix $I - B$, with $I, B \in \mathbb{R}^{N \times N}$ and $B_{ij} \sim \mathcal{N}(0, 0.1)$. For our simulations we choose $N = 4$. As a metric of convergence, we choose the simple MSE between $R_\infty$ and $A^{-1}$.

In our simulation we assume that each memristor is gated by a transistor with a switching time $\tau$. $\tau$ thus determines the delay in both reading and writing. We also assume that during writes, a constant forcing of duration $\theta$ is applied to an element. These dynamics are captured by integrating the matrix differential equation
\begin{equation}
    \dot{R}(t) = -\alpha R(t) + C + G(t) \odot V(t)
\end{equation}
where $G(t) \in \{0, 1\}^{N \times N}$ may be modified as desired to capture different gating and simultaneity constraints.

We first verify that the algorithm converges to the inverse under ideal conditions, i.e. a forcing with $G(t) = \mathbf{1} = J_{n,n}$. The results are shown in Figure \ref{fig:conv_ideal}. The plot on the left is the elementwise evolution of the matrix $R$, i.e. there are 16 plotted trajectories. As expected qualitatively, we see that 4 elements are driven high while the others are allowed to decay. The MSE is as low as 5.42e-5.

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{dde_sim/conv_ideal.png}
    \caption{Convergence under ideal forcing. $\tau = \text{1e-8}$, $\alpha = 0.5, C = 0.001$.}
    \label{fig:conv_ideal}
\end{figure}

We now introduce a non-neglible reading delay $\tau = 1\text{e-3}$. In this situation $G(t)$ is unchanged, but now the corrective forcing $V(t)$ is based on an outdated resistance value. Immediately we observe oscillations (Figure \ref{fig:conv_ideal_delayed}). It is also clear that the oscillations are more severe for the 4 high elements as decay affects them more strongly.

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{dde_sim/conv_ideal_delayed.png}
    \caption{Oscillations emerge with delayed forcing. $\tau = \text{1e-3}$, $\alpha = 0.5, C = 0.001$.}
    \label{fig:conv_ideal_delayed}
\end{figure}

We now consider the ``worst-case" forcing, in which reads are fast but writes must take a substantial time $\tau + \theta$ and only one memristor in the array may be written at a time such that $N^2$ distinct writes are necessary and a complete traversal of the array takes time $N^2(\tau+\theta)$. We observe that the decay of inactive memristors far outpaces any increases in resistances due to driving, precluding convergence to the inverse (Figure \ref{fig:conv_sequential_naive}). Moreover, even with fast reads, significant oscillations occur due to writing delays.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{dde_sim/conv_sequential_naive.png}
    \caption{When writes are sequential with significant writing delays, convergence fails. $\tau = \text{1e-8}$, $\theta = 1\text{e-1}$, $\alpha = 0.5, C = 0.001$.}
    \label{fig:conv_sequential_naive}
\end{figure}

We do expect that the situation improves with an increase in the size of concurrently written subsets. For example, we consider a scheme in which we perform diagonal ``sweeps" of the crossbar with identical writing delays. The situation improves somewhat but not substantially (Figure \ref{fig:conv_diagonal_naive}). The main difference is that there is a slightly greater distinction between ``high" and ``low" elements. In fact our choice of $A$ as diagonally dominant means the following is the best-case scenario, as at least in this situation diagonals approximately share decay progression.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{dde_sim/conv_diagonal_naive.png}
    \caption{A diagonal scheme does not significantly improve the situation. $\tau = \text{1e-8}$, $\theta = 1\text{e-1}$, $\alpha = 0.5, C = 0.001$.}
    \label{fig:conv_diagonal_naive}
\end{figure}

The clear issue is interwrite delays for subsets. To address this, we now apply the adjusted forcing as described in Section \ref{section:compensate}, assuming per-diagonal writes as before.


==> secs/varlearnint.tex <==
\subsection{Variational learning} \textcolor{red}{(if you want to see derivations let me know)}
 We are given samples $\vec x_i\in \mathbb{R}^N$ obtained from a distribution, with well-defined mean and variance. 
 We want to solve the inverse problem for a more  Gaussian ansatz of the form
\begin{eqnarray}
    p(\vec x |A,\vec r)=\frac{1}{Z} e^{-\frac{1}{2} \vec x\ ^t A \vec x+\vec x\ ^t \vec r}.
\end{eqnarray}
for which the mean and variance are sufficient statistics. 

 The KL divergence for this problem, evaluated over the empirical samples, is given by
\begin{eqnarray}
    D_{KL}(p(\vec x)\| p(\vec x |A,\vec r))=\frac{1}{M}\sum_{i=1}^M\Big(-\sum_{ab} \frac{1}{2} (x_i)_a A_{ab} (x_i)_b+\sum_a (x_i)_a r_a\Big)+\log Z(A,\vec r).
\end{eqnarray}
To find the minimum of the KL divergence, we resort to gradient descent, for which the equations are given by
\begin{eqnarray}
    \frac{dA_{ij}}{dt}&=&-\xi \Big(\langle x_i x_j\rangle_{emp}-\big(A^{-1}_{ij}(t) + \mu_i(t) \mu_j(t)\big)\Big) \\
    \frac{dr_i}{dt}&=&-\xi \Big(\langle x_i\rangle_{emp} - \sum_j A^{-1}_{ij}(t) r_j(t)\Big)
\end{eqnarray}
with $\xi$ the learning rate. Above, $\mu_i(t)=\sum_j A^{-1}_{ij}(t) b_i(t)$.

